Quantum thermodynamics in adiabatic open systems and its trapped-ion experimental realization

Quantum thermodynamics aims at investigating both the emergence and the limits of the laws of thermodynamics from a quantum mechanical microscopic approach. In this scenario, thermodynamic processes with no heat exchange, namely, adiabatic transformations, can be implemented through quantum evolutions in closed systems, even though the notion of a closed system is always an idealization and approximation. Here, we begin by theoretically discussing thermodynamic adiabatic processes in open quantum systems, which evolve non-unitarily under decoherence due to its interaction with its surrounding environment. From a general approach for adiabatic non-unitary evolution, we establish heat and work in terms of the underlying Liouville superoperator governing the quantum dynamics. As a consequence, we derive the conditions that an adiabatic open-system quantum dynamics implies in the absence of heat exchange, providing a connection between quantum and thermal adiabaticity. Moreover, we determine families of decohering systems exhibiting the same maximal heat exchange, which imply in classes of thermodynamic adiabaticity in open systems. We then approach the problem experimentally using a hyperfine energy-level quantum bit of an Ytterbium $^{171}$Yb$^+$ trapped ion, which provides a work substance for thermodynamic processes, allowing for the analysis of heat and internal energy throughout a controllable engineered dynamics.

==> table.tex <==
\begin{tabular}{cccccc}
	\multicolumn{1}{l|}{$\gamma_{0}$}         & 314 Hz    & 628 Hz    & 1257 Hz   & 3142 Hz   & 6283 Hz \\ \hline
	\multicolumn{1}{l|}{$\Fcal_{\text{min}}$} & 0.9971(3) & 0.9965(4) & 0.9980(7) & 0.9952(8) & 0.9942(9)
\end{tabular}
